`Keep it Together': Enforcing Cohesion in Extractive Summaries by Simulating Human Memory

Extractive summaries are usually presented as lists of sentences with no expected cohesion between them. In this paper, we aim to enforce cohesion whilst controlling for informativeness and redundancy in summaries, in cases where the input exhibits high redundancy. The pipeline controls for redundancy in long inputs as it is consumed, and balances informativeness and cohesion during sentence selection. Our sentence selector simulates human memory to keep track of topics --modeled as lexical chains--, enforcing cohesive ties between noun phrases. Across a variety of domains, our experiments revealed that it is possible to extract highly cohesive summaries that nevertheless read as informative to humans as summaries extracted by only accounting for informativeness or redundancy. The extracted summaries exhibit smooth topic transitions between sentences as signaled by lexical chains, with chains spanning adjacent or near-adjacent sentences.

==> backup.tex <==
%% notes trimmed from main doc

% \subsection{Matching the Similarity Distribution}

% Following previous work \cite{xiao2020systematically,qian2019reducing}, we model the trade-off between informativeness and cohesiveness by defining the score of sentence $s_i$, $f(s_i)$, as
% \begin{equation}
% \label{eq:emb-trade}
%     f(s_i) = \lambda_{sel} f_{inf}(s_i) - (1-\lambda_{sel}) f_{coh}(\hat{S}^i)
% \end{equation}
% \noindent where function $f_{inf}(\cdot)$ estimates the informativeness of $s_i$ and 
% $f_{coh}(\cdot)$ estimates the cohesiveness of candidate summary $\hat{S}^i$, and $\lambda_{sel} \in [0,1]$ is a parameter that allows controlling for their trade-off.
% In this work, we take the probability of selecting $s_i$ given by model $M$ as a proxy for informativeness, i.e.\
% $f_{inf}(s_i)=p(y_i|s_i;\Theta)$.
% Finally, the optimal selection is defined as $s_i^*=\argmax_{s_i \in D \setminus \hat{S} } f(s_i)$.

% In order to formulate $f_{coh}(\cdot)$, we analysed the distribution of cosine similarity between embeddings of content units in reference summaries. % and found that it follows a Normal distribution.
% Intuitively, a well-written, cohesiveness text, the semantic similarity of a sentence against nearby sentences follows a sharp decreasing gradient,
% with immediately adjacent sentences being the most similar.
% Based on this insight, we propose sentence selectors that aim to extract candidate summaries that best emulate this similarity distribution.


\paragraph{Distance from Mean Similarity (Dist-Sim).}
This selector models cohesiveness as the difference between means of the inter-sentential similarity distributions of reference summaries and candidate summaries.
Formally, 
\begin{equation*}
f_{coh}=-|\bar{\mu}_{sim} - \mu_{sim}^{i} |    
\end{equation*}
\noindent where $\bar{\mu}_{sim}$ is the mean pairwise cosine similarity between sentences in reference summaries.
In practice, we precalculate $\bar{\mu}_{sim}$ and keep it constant throughout our experiments.
Similarly, $\mu_{sim}^{i}$ is the mean similarity in the candidate summary, including $s_i$, defined as
\begin{equation*}
 \mu_{sim}^{i}=\mean_{x,y \in \hat{S}^i, x \neq y} Sim(x,y)   
\end{equation*}
\noindent where $Sim(\cdot)$ indicates cosine similarity between sentence embeddings.
Intuitively, \textsc{Dist-Sim} will encourage the extraction of candidate summaries with average inter-sentential similarity 
similar to the average similarity seen in reference summaries.


\paragraph{Distance from Mean Similarity Gap  (Dist-Gap).}
Next, we investigated the distribution of maximal similarity gaps, i.e.\ the difference between the maximum and minimum similarity scores between sentence embeddings in a candidate summary.
Given that this distribution was also found to be Normal, we define 
$f_{coh}=|\bar{\mu}_{gap} - \mu_{gap}^{i} |$, where $\mu_{gap}^{i}$ is defined as 
\begin{equation*}
 \mu_{gap}^{i}=\max_{x,y \in \hat{S}^i, x \neq y} Sim(x,y) - \min_{x,y \in \hat{S}^i, x \neq y} Sim(x,y)
\end{equation*}
\noindent and $\bar{\mu}_{gap}$ is precalculated over reference summaries.


